StructDiffusion: Language-Guided Creation of Physically-Valid Structures using Unseen Objects

Robots operating in human environments must be able to rearrange objects into semantically-meaningful configurations, even if these objects are previously unseen. In this work, we focus on the problem of building physically-valid structures without step-by-step instructions. We propose StructDiffusion, which combines a diffusion model and an object-centric transformer to construct structures given partial-view point clouds and high-level language goals, such as "set the table". Our method can perform multiple challenging language-conditioned multi-step 3D planning tasks using one model. StructDiffusion even improves the success rate of assembling physically-valid structures out of unseen objects by on average 16% over an existing multi-modal transformer model trained on specific structures. We show experiments on held-out objects in both simulation and on real-world rearrangement tasks. Importantly, we show how integrating both a diffusion model and a collision-discriminator model allows for improved generalization over other methods when rearranging previously-unseen objects. For videos and additional results, see our website: https://structdiffusion.github.io/.

==> 05data_gen.tex <==
\begin{figure}[bt]
\includegraphics[width=1.0\columnwidth]{figures/housekeep_custom_objects.png}
\centering
\caption{
Testing objects from Google Scanned Objects~\cite{downs2022google}, ReplicaCAD dataset~\cite{szot2021habitat}, and YCB object Set~\cite{calli2015ycb}. The test object dataset contains a wide range of textured objects belonging to various classes. None of these objects appear in the training data.
}
\label{fig:objects}
\end{figure}

==> intro-figure.tex <==
\setcounter{figure}{1}
\makeatletter
\let\@oldmaketitle\@maketitle% Store \@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle% Update \@maketitle to insert...
  \begin{center}
    \includegraphics[width=0.83\linewidth]
    {figures/examples.pdf}
  \end{center}
  %\refstepcounter{figure}
  \vspace{-6pt}
  \footnotesize{\textbf{Fig.~\thefigure:\label{fig:intro-example}}~StructFormer rearranges unknown objects into semantically meaningful spatial structures based on high-level language instructions and partial-view point cloud observations of the scene. The model use multi-modal transformers to predict both which objects to manipulate and where to place them.}% CAPTION
 \vspace{-24pt}
  \medskip}% ... an image
\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "00draft"
%%% End:

